Towards Learning Contrast Kinetics with Multi-Condition Latent Diffusion Models

Contrast agents in dynamic contrast enhanced magnetic resonance imaging allow to localize tumors and observe their contrast kinetics, which is essential for cancer characterization and respective treatment decision-making. However, contrast agent administration is not only associated with adverse health risks, but also restricted for patients during pregnancy, and for those with kidney malfunction, or other adverse reactions. With contrast uptake as key biomarker for lesion malignancy, cancer recurrence risk, and treatment response, it becomes pivotal to reduce the dependency on intravenous contrast agent administration. To this end, we propose a multi-conditional latent diffusion model capable of acquisition time-conditioned image synthesis of DCE-MRI temporal sequences. To evaluate medical image synthesis, we additionally propose and validate the Fr\'echet radiomics distance as an image quality measure based on biomarker variability between synthetic and real imaging data. Our results demonstrate our method's ability to generate realistic multi-sequence fat-saturated breast DCE-MRI and uncover the emerging potential of deep learning based contrast kinetics simulation. We publicly share our accessible codebase at https://github.com/RichardObi/ccnet and provide a user-friendly library for Fr\'echet radiomics distance calculation at https://pypi.org/project/frd-score.

==> Figures/scatter-idc-curves.tex <==
%\newcommand{\rulesep}{\unskip\ \vrule\ }


\begin{figure}[htb]
    \begin{subfigure}{.5\textwidth}
    \centering
    \caption[]{3T IDC Curve}    
    \begin{tikzpicture}[scale=0.86,transform shape]
    \centering
      %\pgfplotsset{
      %    scale only axis,
      %}
       \begin{axis}[enlargelimits=0.05, 
            %xmode=log,
            %ymode=log,
            log ticks with fixed point,
            %xtick=\empty,
            %axis x line=center,
            %axis y line=center,
            xlabel=seconds since precontrast acquisition,
            %ylabel=mean pixel intensity,
            grid=both,
            %ylabel near ticks,
            %xlabel near ticks,
            scale only axis=true,
            width=1.0\textwidth, %15cm,
            height=1.0\textwidth, %4.5cm,
            %height=1.165\textwidth, %4.5cm,
            ytick={0, 50, 100, 150, 200, 250},
            xtick={0, 200, 400, 600, 800, 1000, 1200},
            ymin=0, %70, %0,
            xmax=255,
            ymin=0,
            xmax=1200,
            %legend style={font=\small},
            legend cell align=left,
            legend pos=north west %south east
        ]
        \addplot+ [mark=*, color=blue][
            scatter/classes={c={mark=square*, mark options={line width=0.55pt}, draw=black, fill=blue}}, %{a={blue}, b={orange}},%, c={green}, d={orange}}, %, e={yellow}, f={red}, g={black}, h={gray}, i={brown}},
            scatter, mark=*, only marks, sharp plot,
            scatter src=explicit symbolic,
            nodes near coords*={\Label},
            visualization depends on={value \thisrow{label} \as \Label}
            % a = Gaussian Noise
            % b = Gaussian Blur
        ] table [meta=class] {
            x y class label
            0 10 c \footnotesize{ABC}
            200 150 c \footnotesize{ABC}
            400 160 c \footnotesize{ABC} 
            600 200 c \footnotesize{ABC}  
            800 110 c \footnotesize{ABC} 
            1000 80 c \footnotesize{ABC}  
            1200 20 c \footnotesize{ABC}  
        };
        \addplot+ [mark=*, color=blue][
            scatter/classes={c={mark=square*, mark options={line width=0.55pt}, draw=black, fill=blue}}, %{a={blue}, b={orange}},%, c={green}, d={orange}}, %, e={yellow}, f={red}, g={black}, h={gray}, i={brown}},
            %scatter/classes={a={blue}, b={orange}},%, c={green}, d={orange}}, %, e={yellow}, f={red}, g={black}, h={gray}, i={brown}},
            scatter, mark=*, only marks, sharp plot, densely dashed,
            scatter src=explicit symbolic,
            nodes near coords*={\Label},
            visualization depends on={value \thisrow{label} \as \Label}
            % a = Gaussian Noise
            % b = Gaussian Blur
        ] table [meta=class] {
            x y class label
            0 10 c \footnotesize{ABC}
            200 130 c \footnotesize{ABC}
            400 190 c \footnotesize{ABC} 
            600 240 c \footnotesize{ABC}  
            800 200 c \footnotesize{ABC} 
            1000 150 c \footnotesize{ABC}  
            1200 110 c \footnotesize{ABC}  
        };
        \addplot+ [mark=*, color=orange][
            scatter/classes={b={mark=pentagon*, mark options={line width=0.55pt}, draw=black, fill=orange}}, %{a={blue}, b={orange}},%, c={green}, d={orange}}, %, e={yellow}, f={red}, g={black}, h={gray}, i={brown}},
            scatter, mark=*, only marks, sharp plot,
            scatter src=explicit symbolic,
            nodes near coords*={\Label},
            visualization depends on={value \thisrow{label} \as \Label}
            % a = Gaussian Noise
            % b = Gaussian Blur
        ] table [meta=class] {
            x y class label
            0 20 b \footnotesize{ABC}
            200 120 b \footnotesize{ABC}
            400 170 b \footnotesize{ABC} 
            600 205 b \footnotesize{ABC}  
            800 205 b \footnotesize{ABC} 
            1000 190 b \footnotesize{ABC}  
            1200 20 b \footnotesize{ABC}  
        };
        \addplot+ [mark=*, color=orange][
            scatter/classes={b={mark=pentagon*, mark options={line width=0.55pt}, draw=black, fill=orange}}, %{a={blue}, b={orange}},%, c={green}, d={orange}}, %, e={yellow}, f={red}, g={black}, h={gray}, i={brown}},
            %scatter/classes={a={blue}, b={orange}},%, c={green}, d={orange}}, %, e={yellow}, f={red}, g={black}, h={gray}, i={brown}},
            scatter, mark=*, only marks, sharp plot, densely dashed,
            scatter src=explicit symbolic,
            nodes near coords*={\Label},
            visualization depends on={value \thisrow{label} \as \Label}
            % a = Gaussian Noise
            % b = Gaussian Blur
        ] table [meta=class] {
            x y class label
            0 15 b \footnotesize{ABC}
            200 160 b \footnotesize{ABC}
            400 170 b \footnotesize{ABC} 
            600 200 b \footnotesize{ABC}  
            800 210 b \footnotesize{ABC} 
            1000 200 b \footnotesize{ABC}  
            1200 10 b \footnotesize{ABC}  
        };
    \legend{\footnotesize{Case233},,\footnotesize{Case192}}
    \end{axis}
    \end{tikzpicture} 
    %\caption[]{}
    %\label{fig:FRD}
    \end{subfigure}
    \hfill 
    %\rulesep
    %\vspace{-10pt}
    %\break
    \begin{subfigure}{.5\textwidth}
    %\centering
    \captionsetup{justification=centering}
    \caption[]{1.5T IDC Curve}
    \begin{tikzpicture}[scale=0.86,transform shape]
    \centering
      %\pgfplotsset{
      %    scale only axis,
      %}
           \begin{axis}[enlargelimits=0.05, 
            %xmode=log,
            %ymode=log,
            log ticks with fixed point,
            %xtick=\empty,
            %axis x line=center,
            %axis y line=center,
            xlabel=seconds since precontrast acquisition,
            %ylabel=mean pixel intensity,
            grid=both,
            %ylabel near ticks,
            %xlabel near ticks,
            scale only axis=true,
            width=1.0\textwidth, %15cm,
            height=1.0\textwidth, %4.5cm,
            %height=1.165\textwidth, %4.5cm,
            ytick={0, 50, 100, 150, 200, 250},
            xtick={0, 200, 400, 600, 800, 1000, 1200},
            ymin=0, %70, %0,
            xmax=255,
            ymin=0,
            xmax=1200,
            %legend style={font=\small},
            legend cell align=left,
            legend pos=north west %south east
        ]
        \addplot+ [mark=*, color=gray][
            scatter/classes={c={mark=square*, mark options={line width=0.55pt}, draw=black, fill=gray}}, %{a={blue}, b={orange}},%, c={green}, d={orange}}, %, e={yellow}, f={red}, g={black}, h={gray}, i={brown}},
            scatter, mark=*, only marks, sharp plot,
            scatter src=explicit symbolic,
            nodes near coords*={\Label},
            visualization depends on={value \thisrow{label} \as \Label}
            % a = Gaussian Noise
            % b = Gaussian Blur
        ] table [meta=class] {
            x y class label
            0 50 c \footnotesize{ABC}
            200 150 c \footnotesize{ABC}
            400 160 c \footnotesize{ABC} 
            600 190 c \footnotesize{ABC}  
            800 110 c \footnotesize{ABC} 
            1000 90 c \footnotesize{ABC}  
            1200 30 c \footnotesize{ABC}  
        };
        \addplot+ [mark=*, color=gray][
            scatter/classes={c={mark=square*, mark options={line width=0.55pt}, draw=black, fill=gray}}, %{a={blue}, b={orange}},%, c={green}, d={orange}}, %, e={yellow}, f={red}, g={black}, h={gray}, i={brown}},
            %scatter/classes={a={blue}, b={orange}},%, c={green}, d={orange}}, %, e={yellow}, f={red}, g={black}, h={gray}, i={brown}},
            scatter, mark=*, only marks, sharp plot, densely dashed,
            scatter src=explicit symbolic,
            nodes near coords*={\Label},
            visualization depends on={value \thisrow{label} \as \Label}
            % a = Gaussian Noise
            % b = Gaussian Blur
        ] table [meta=class] {
            x y class label
            0 60 c \footnotesize{ABC}
            200 150 c \footnotesize{ABC}
            400 190 c \footnotesize{ABC} 
            600 230 c \footnotesize{ABC}  
            800 210 c \footnotesize{ABC} 
            1000 150 c \footnotesize{ABC}  
            1200 110 c \footnotesize{ABC}  
        };
        \addplot+ [mark=*, color=red][
            scatter/classes={b={mark=pentagon*, mark options={line width=0.55pt}, draw=black, fill=red}}, %{a={blue}, b={orange}},%, c={green}, d={orange}}, %, e={yellow}, f={red}, g={black}, h={gray}, i={brown}},
            scatter, mark=*, only marks, sharp plot,
            scatter src=explicit symbolic,
            nodes near coords*={\Label},
            visualization depends on={value \thisrow{label} \as \Label}
            % a = Gaussian Noise
            % b = Gaussian Blur
        ] table [meta=class] {
            x y class label
            0 25 b \footnotesize{ABC}
            200 130 b \footnotesize{ABC}
            400 140 b \footnotesize{ABC} 
            600 215 b \footnotesize{ABC}  
            800 225 b \footnotesize{ABC} 
            1000 120 b \footnotesize{ABC}  
            1200 110 b \footnotesize{ABC}  
        };
        \addplot+ [mark=*, color=red][
            scatter/classes={b={mark=pentagon*, mark options={line width=0.55pt}, draw=black, fill=red}}, %{a={blue}, b={orange}},%, c={green}, d={orange}}, %, e={yellow}, f={red}, g={black}, h={gray}, i={brown}},
            %scatter/classes={a={blue}, b={orange}},%, c={green}, d={orange}}, %, e={yellow}, f={red}, g={black}, h={gray}, i={brown}},
            scatter, mark=*, only marks, sharp plot, densely dashed,
            scatter src=explicit symbolic,
            nodes near coords*={\Label},
            visualization depends on={value \thisrow{label} \as \Label}
            % a = Gaussian Noise
            % b = Gaussian Blur
        ] table [meta=class] {
            x y class label
            0 15 b \footnotesize{ABC}
            200 130 b \footnotesize{ABC}
            400 170 b \footnotesize{ABC} 
            600 240 b \footnotesize{ABC}  
            800 230 b \footnotesize{ABC} 
            1000 210 b \footnotesize{ABC}  
            1200 190 b \footnotesize{ABC}  
        };
    \legend{\footnotesize{Case009},,\footnotesize{Case120}}
    \end{axis}
    \end{tikzpicture} 
    %\caption[]{}
    %\label{fig:FRD}
    \end{subfigure}
\caption[]{IDC curves of test set cases for synthetic (dashed lines) and real (solid lines) images of single tumor-containing breasts. Intensity values (y-axis) per time point (x-axis) are computed as the mean of intensity values of tumor containing pixels per image according to ground truth masks. The testset cases are stratified per field strength into 1.5T and 3T acquisitions.
} 
\label{fig:IDC}
\end{figure}
